DocVLM: Make Your VLM an Efficient Reader

Vision-Language Models (VLMs) excel in diverse visual tasks but face challenges in document understanding, which requires fine-grained text processing. While typical visual tasks perform well with low-resolution inputs, reading-intensive applications demand high-resolution, resulting in significant computational overhead. Using OCR-extracted text in VLM prompts partially addresses this issue but underperforms compared to full-resolution counterpart, as it lacks the complete visual context needed for optimal performance. We introduce DocVLM, a method that integrates an OCR-based modality into VLMs to enhance document processing while preserving original weights. Our approach employs an OCR encoder to capture textual content and layout, compressing these into a compact set of learned queries incorporated into the VLM. Comprehensive evaluations across leading VLMs show that DocVLM significantly reduces reliance on high-resolution images for document understanding. In limited-token regimes (448$\times$448), DocVLM with 64 learned queries improves DocVQA results from 56.0% to 86.6% when integrated with InternVL2 and from 84.4% to 91.2% with Qwen2-VL. In LLaVA-OneVision, DocVLM achieves improved results while using 80% less image tokens. The reduced token usage allows processing multiple pages effectively, showing impressive zero-shot results on DUDE and state-of-the-art performance on MP-DocVQA, highlighting DocVLM's potential for applications requiring high-performance and efficiency.

==> tables/attn_maps_abl.tex <==


\begin{table}[ht]
\centering
\tablefontsize
\begin{tabularx}{\tablewidth}{@{}l@{\hspace{0.3em}}c@{\hspace{0.5em}}c@{\hspace{0.2em}}|ccc@{}}
\toprule
Method &  Enc & Causal & DocVQA & InfoVQA & OCR-VQA \\
\midrule
\multirow{2}{*}{Baseline} & \multirow{2}{*}{$\times$} & $\checkmark$ & 76 \textbar{} 79 & 47 \textbar{} 48 & ? \textbar{} ? \\
 &  &  $\times$ & 74 \textbar{} 79 & 42 \textbar{} 48 & ? \textbar{} ? \\
\midrule
\multirow{2}{*}{PrefixLM} & \multirow{2}{*}{$\checkmark$} & $\checkmark$ & 83 \textbar{} 87 & 44 \textbar{} 59 & ? \textbar{} ? \\
 &  &  $\times$ & \textbf{86} \textbar{} \textbf{88} & \textbf{54} \textbar{} \textbf{60} & ? \textbar{} ? \\
\bottomrule
\end{tabularx}
\caption{Comparison of methods for Causal vs. Non-causal Attention. Test results are shown as X\textbar{}Y, where X is the score on the partial training set and Y is the score on the full training set. The metrics used are ANLS for DocVQA and InfoVQA, and EM for OCR-VQA.}
\label{tab:causal_noncausal}
\end{table}

==> tables/comparison_pretraining_tab.tex <==


\begin{table}[ht]
\centering
\tablefontsize
\begin{tabularx}{\tablewidth}{@{}l@{\hspace{0.3em}}c@{\hspace{0.5em}}c@{\hspace{0.2em}}|ccc@{}}
\toprule
Method & Fusion & PT & DocVQA & InfoVQA & OCR-VQA \\
\midrule
\multirow{2}{*}{PrefixLM} & \multirow{2}{*}{Input} & $\times$ & 86 \textbar{} 88 & 54 \textbar{} 60 & ? \textbar{} ? \\
 &   & $\checkmark$ & \textbf{87} \textbar{} \textbf{89} & \textbf{58} \textbar{} \textbf{63} & ? \textbar{} ? \\
\midrule
\multirow{2}{*}{DocMistral} & \multirow{2}{*}{CA} & $\times$ & 79 \textbar{} 85 & 44 \textbar{} 51 & ? \textbar{} ? \\
 &  & $\checkmark$ & 85 \textbar{} 86 & 50 \textbar{} 54 & ? \textbar{} ? \\
\bottomrule
\end{tabularx}
\caption{Comparison of methods and their performance with and without pretraining. Test results are shown as X\textbar{}Y, where X is the score on the partial training set and Y is the score on the full training set. The metrics used are ANLS for DocVQA and InfoVQA, and EM for OCR-VQA.}
\label{tab:comparison_pretraining}
\end{table}

==> tables/compression_abla_lavva.tex <==


\begin{table*}[h]
\centering
\tablefontsize
\caption{Results on Llava One-Vision on DocVQA \mnote{Val?} without changing Llava's weights}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{AnyRes Max}} & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{c|}{\textbf{+ OCR encoder}} & \multicolumn{2}{c|}{\textbf{+ Q-OCR encoder}} \\
& \textbf{Score} & \textbf{Max Visual Tokens} & \textbf{Score} & \textbf{Max OCR Tokens} & \textbf{Score} & \textbf{Q-OCR Tokens} \\ \hline
\textbf{1} & 0.6626 & 1,458 & 0.8924 & 800 & 0.8384 & 64 \\ \hline
 % & 0.8384 & \multicolumn{2}{c|}{} & 64 \\ \hline
\textbf{2} & 0.7512 & 2,187 & 0.8952 & 800  & 0.8515 & 64 \\ \hline
% \textbf{+ Q-OCR tokens} & 0.8515 & \multicolumn{2}{c|}{} & 64 \\ \hline
\textbf{3} & 0.8086 & 2,916 & 0.9003 & 800 & 0.8662 & 64 \\ \hline
\textbf{4} & 0.8384 & 3,645 & 0.9082 & 800 & 0.8793 & 64 \\ \hline
\textbf{5} & 0.8517 & 4,374 & 0.9093 & 800 & 0.8855 & 64 \\ \hline
\textbf{6} & 0.8626 & 5,103 & 0.9087 & 800 & 0.8895 & 64 \\ \hline
\textbf{7} & 0.8652 & 5,842 & 0.9082 & 800 & 0.8908 & 64 \\ \hline
\textbf{8} & 0.8694 & 6,561 & 0.9085 & 800 & 0.8926 & 64 \\ \hline
\textbf{9} & 0.8717 & 7,290 & 0.9058 & 800 & 0.8920 & 64 \\ \hline
\end{tabular}
\end{table*}


==> tables/integration_strategies_figure.tex <==
\begin{figure}[t] 
  \centering
  \includegraphics[width=0.98\linewidth]{figures/llm_vs_pre_vs_ca_v3.pdf}
  \caption{\textbf{Comparison of Various Integration Strategies}.
We examine different strategies for integrating OCR information, including causal, non-causal, and cross-attention approaches.
}
    \label{fig:integration_strategies}
\end{figure}

==> tables/llm_table_results.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c c}
 \cmidrule[1pt](){1-7}
\textbf{Model} & \textbf{Enc.} & \textbf{Integration} & \textbf{LoRA} & \textbf{Compression} & {DocVQA} & {InfoVQA} \\
 \cmidrule(){1-7}

 \multicolumn{7}{c}{\textbf{Baselines}} \\
 \cmidrule(){1-7}
\textcolor{gray}{LayoutLM-LARGE} & \textcolor{gray}{$\times$} & \textcolor{gray}{Latin prompt} & \textcolor{gray}{$\times$} & \textcolor{gray}{-} & \textcolor{gray}{72.6} & \textcolor{gray}{27.2} \\
\textcolor{gray}{Claude-V1.3} & \textcolor{gray}{$\times$} & \textcolor{gray}{Latin prompt} & \textcolor{gray}{$\times$} & \textcolor{gray}{-} & \textcolor{gray}{83.4} & \textcolor{gray}{54.5} \\
\textcolor{gray}{ChatGPT-3.5} & \textcolor{gray}{$\times$} & \textcolor{gray}{Latin prompt} & \textcolor{gray}{$\times$} & \textcolor{gray}{-} & \textcolor{gray}{82.6} & \textcolor{gray}{49.0} \\
\textcolor{gray}{DocLLM} & \textcolor{gray}{$\checkmark$} & \textcolor{gray}{Causal} & \textcolor{gray}{-} & \textcolor{gray}{$\times$} & \textcolor{gray}{69.5} & \textcolor{gray}{-} \\
 \cmidrule(){1-7}

 \multicolumn{7}{c}{\textbf{Base Model: Mistral}} \\
 \cmidrule(){1-7}
Mistral & $\times$ & Causal & $\checkmark$ & $\times$ & 79.1 & 48.1 \\
Mistral & $\checkmark$ & CA & $\checkmark$ & $\times$ & 84.8 & 51.2 \\
Mistral & $\checkmark$ & CA+Pretrain & $\checkmark$ & $\times$ & 86.2 & 54.1 \\
Mistral & $\checkmark$ & Prefix & $\times$ & $\times$ & 86.6 & 59.2 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Causal & $\times$ & $\times$ & 85.0 & 56.3 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Causal & $\checkmark$ & $\times$ & 87.4 & 59.4 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Causal & $\times$ & $\checkmark$ & 81.2 & 52.8 \\
 \cmidrule(){1-7}

 \multicolumn{7}{c}{\textbf{Base Model: Qwen2}} \\
 \cmidrule(){1-7}
Qwen2 & $\times$ & Input & - & - & 76.4 & 44.5 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Prefix & $\times$ & $\times$ & 89.2 & 62.8 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Causal & $\times$ & $\times$ & 89.2 & 62.9 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Prefix & $\times$ & $\checkmark$ & 85.4 & 55.8 \\
\textbf{\ourmethod (Ours)} & $\checkmark$ & Causal & $\times$ & $\checkmark$ & 85.5 & 56.8 \\
\cmidrule[1pt](){1-7}
\end{tabular}}
\caption{\textbf{Comparison in OCR-Only Setting.} We assess our method’s performance when integrated solely with LLMs, without using the vision modality. Results demonstrate that our method significantly enhances performance even in this configuration.\label{tab:llm_intergration}}
\end{table}










==> tables/ocr_integration_abl.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{
%  \cmidrule[1pt](){1-7}
% \begin{table}[ht]
% \centering
% \resizebox{\linewidth}{!}{
% \renewcommand{\arraystretch}{1.3} % Adjust row height for readability
% \begin{tabular}{l c c c c c  c c }
% \toprule
% \textbf{Enc.} & \textbf{LoRa} & \textbf{Vis-align.} & \textbf{Compress.} & \textbf{Attn.} & \textbf{DocVQA} & \textbf{InfoVQA} \\
% \midrule
% \multirow{2}{*}{$\times$} & $\times$ & $\times$ & $\times$ & \multirow{8}{*}{Casual} & ? & ?  \\
%  & $\checkmark$ & $\times$ & $\times$ &  & ? & ?  \\
% \multirow{6}{*}{$\checkmark$} & $\times$ & $\times$ & $\times$ &  & ? & ?  \\
%  & $\times$ & $\checkmark$ & $\times$ &  & ? & ?  \\
%  & $\checkmark$ & $\checkmark$ & $\times$ &  & ? & ?  \\
%  & $\times$ & $\times$ & $\checkmark$ &  & ? & ?  \\
%  & $\times$ & $\checkmark$ & $\checkmark$ &  & ? & ?  \\
%  & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & ? & ?  \\
% \cdashline{1-7} & \\[-2ex]
% \multirow{2}{*}{$\times$} & $\times$ & $\times$ & $\times$ & \multirow{8}{*}{Prefix} & ? & ?  \\
%  & $\checkmark$ & $\times$ & $\times$ &  & ? & ?  \\
% \multirow{6}{*}{$\checkmark$} & $\times$ & $\times$ & $\times$ &  & ? & ?  \\
%  & $\times$ & $\checkmark$ & $\times$ &  & ? & ?  \\
%  & $\checkmark$ & $\checkmark$ & $\times$ &  & ? & ?  \\
%  & $\times$ & $\times$ & $\checkmark$ &  & ? & ?  \\
%  & $\times$ & $\checkmark$ & $\checkmark$ &  & ? & ?  \\
%  & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & ? & ?  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison across OCR fusion strategies, training stages, and the use of non-causal attention map (PrefixLM).}
% \label{tab:ocr_fusion_comparison}
% \end{table}

\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.3} % Adjust row height for readability
\begin{tabular}{c | l c c c | c c}
\toprule
\textbf{Attn.} & \textbf{Enc.} & \textbf{Vis-align.} & \textbf{LoRA} & \textbf{Compress.} & \textbf{DocVQA} & \textbf{InfoVQA} \\
\midrule
\multirow{8}{*}{\rotatebox{90}{Casual}} & $\times$ & $\times$ & $\times$ & $\times$ & 89.1 & 55.6 \\
 & $\times$ & $\times$ & $\checkmark$ & $\times$ & 90.8 & 60.8 \\
 & $\checkmark$ & $\times$ & $\times$ & $\times$ & 91.9 & \textbf{65.3} \\
 & $\checkmark$ & $\checkmark$ & $\times$ & $\times$ & 92.0 & 65.0 \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$ & \textbf{92.3} & 64.7 \\
 & $\checkmark$ & $\times$ & $\times$ & $\checkmark$ & 90.2 & 60.2 \\
 & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & 91.2 & 61.2 \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 91.2 & 61.2 \\
\cmidrule{2-7}
\multirow{7}{*}{\rotatebox{90}{Prefix}} & $\times$ & $\times$ & $\times$ & $\times$ &  &  \\
 & $\checkmark$ & $\times$ & $\times$ & $\times$ & 91.1 & 63.5 \\
 & $\checkmark$ & $\checkmark$ & $\times$ & $\times$ & 91.0 & 64.3 \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$ & ? & ? \\
 & $\checkmark$ & $\times$ & $\times$ & $\checkmark$ & 67.5 & 38.8 \\
 & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & ? & ? \\
 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & ? & ? \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison across OCR fusion strategies, training stages, and the use of non-causal attention map (PrefixLM).}
\label{tab:ocr_fusion_comparison}
\end{table}








% \begin{table}[ht]
% \centering
% \begin{tabularx}{\linewidth}{l c | c c}
% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l c c | c c }
%  \cmidrule[1pt](){1-5}
% \textbf{OCR Fusion} & \textbf{Enc} & \textbf{Pre-Training} & \textbf{DocVQA} & \textbf{InfoVQA} \\
%  \cmidrule(){1-5}
% Text & $\times$ & $\times$  & 79 & 48 \\
% Cross-Attention & $\checkmark$ & $\times$ & 85 & 51 \\
% Cross-Attention & $\checkmark$ & $\checkmark$ & 86 & 54 \\
% \methodname & $\checkmark$ & $\times$ & \textbf{87} & \textbf{59} \\
% \methodname & $\checkmark$ & $\checkmark$ & \textbf{?} & \textbf{?} \\
% \cmidrule[1pt](){1-5}
% \end{tabular}
% }
% \caption{\textbf{OCR Integration and Pre-training.}
% We ablate the .}
% \label{tab:llm_intergration}
% \end{table}
% \bottomrule
% \end{tabularx}
% \caption{Comparison of OCR integration strategies and OCR information fusion techniques for Mistral model. \mnote{Need to make the table more compact and clear.}}
% \label{tab:ocr_integration_strategies}
% \end{table}




% \begin{table}[ht]
% \centering
% \tablefontsize
% \begin{tabularx}{\tablewidth}{@{}l@{\hspace{0.3em}}c@{\hspace{0.5em}}c@{\hspace{0.2em}}|ccc@{}}
% \toprule
% Method  & Fusion & Enc & DocVQA & InfoVQA & OCR-VQA \\
% \midrule
% Baseline  & Input & $\times$ & 76 \textbar{} 79 & 47 \textbar{} 48 & ? \textbar{} ? \\
% PrefixLM  & Input & $\checkmark$ & \textbf{86} \textbar{} \textbf{88} & \textbf{54} \textbar{} \textbf{60} & ? \textbar{} ? \\
% DocMistral  & CA & $\checkmark$ & 79 \textbar{} 85 & 44 \textbar{} 51 & ? \textbar{} ? \\
% \bottomrule
% \end{tabularx}
% \caption{Comparison of methods with OCR integration strategies and OCR information fusion techniques. Test results are shown as X\textbar{}Y, where X is the score on the partial training set and Y is the score on the full training set. The metrics used are ANLS for DocVQA and InfoVQA, and EM for OCR-VQA. \mnote{Need to mention this is without pretraining in the transition to the next section. Change all tables to two columns for val and test.}}
% \end{table}


% \begin{table}[ht]
% \centering
% \tablefontsize
% \begin{tabularx}{\tablewidth}{lc|cccccc}
% \toprule
% Method  & Enc & \multicolumn{2}{c}{DocVQA} & \multicolumn{2}{c}{InfoVQA} & \multicolumn{2}{c}{OCR-VQA} \\
% & & P & F & P & F & P & F\\
% \midrule
% Baseline & $\times$ & 76 & 79 & 47 & 48 & ? & ? \\
% Decoder-only & $\checkmark$ & 86 & 88 & 54 & 60 & ? & ? \\
% CA & $\checkmark$ & 79 & 85 & 44 & 51 & ? & ? \\
% \bottomrule
% \end{tabularx}
% \caption{Comparison of methods with OCR integration strategies and OCR information fusion techniques. Test results are shown as X\textbar{}Y, where X is the score on the partial training set and Y is the score on the full training set. The metrics used are ANLS for DocVQA and InfoVQA, and EM for OCR-VQA. \mnote{Need to mention this is without pretraining in the transition to the next section. Change all tables to two columns for val and test.}}
% \end{table}


==> tables/training_datasets_table_with_partial.tex <==

\begin{table}[ht]
\centering
\tablefontsize
\begin{tabularx}{\tablewidth}{@{}l@{\hspace{\tablehspace}}l@{\hspace{\tablehspace}}c@{\hspace{\tablehspace}}c@{}}
\toprule
\textbf{Category} & \textbf{Dataset} & \textbf{Partial} & \textbf{Full} \\
\midrule
\multirow{4}{*}{Document QA} & DocVQA      & $\checkmark$ & $\checkmark$ \\
                             & InfoVQA     & $\checkmark$ & $\checkmark$ \\
                             & ChartQA     & $\checkmark$ & $\checkmark$ \\
                             & TAT-DQA     & $\times$ & $\checkmark$ \\
\midrule
\multirow{2}{*}{Scene Text}  & TextVQA     & $\times$ & $\checkmark$ \\
                             & OCR-VQA     & $\times$ & $\checkmark$ \\
\midrule
\multirow{1}{*}{Captioning}  & TextCaps    & $\times$ & $\checkmark$ \\
\midrule
\textbf{Total Examples} & & \textbf{XX,XXX} & \textbf{XXX,XXX} \\
\bottomrule
\end{tabularx}
\caption{Training dataset configurations for "Partial" and "Full" settings, categorized by Document QA, Scene Text, and Captioning datasets. A checkmark ($\checkmark$) indicates the dataset is included, while a cross ($\times$) means it is not. The total number of training examples for each configuration is shown at the bottom. \mnote{This is only relevant to the prefix experiments which I'm not sure we will have. Anyway the datasets table should move to the appendix.}}
\label{tab:training_datasets}
\end{table}
